The Power of Perception in Human-AI Interaction: Investigating Psychological Factors and Cognitive Biases that Shape User Belief and Behavior

This thesis investigates the psychological factors that influence belief in AI predictions, comparing them to belief in astrology- and personality-based predictions, and examines the "personal validation effect" in the context of AI, particularly with Large Language Models (LLMs). Through two interconnected studies involving 238 participants, the first study explores how cognitive style, paranormal beliefs, AI attitudes, and personality traits impact perceptions of the validity, reliability, usefulness, and personalization of predictions from different sources. The study finds a positive correlation between belief in AI predictions and belief in astrology- and personality-based predictions, highlighting a "rational superstition" phenomenon where belief is more influenced by mental heuristics and intuition than by critical evaluation. Interestingly, cognitive style did not significantly affect belief in predictions, while paranormal beliefs, positive AI attitudes, and conscientiousness played significant roles. The second study reveals that positive predictions are perceived as significantly more valid, personalized, reliable, and useful than negative ones, emphasizing the strong influence of prediction valence on user perceptions. This underscores the need for AI systems to manage user expectations and foster balanced trust. The thesis concludes with a proposal for future research on how belief in AI predictions influences actual user behavior, exploring it through the lens of self-fulfilling prophecy. Overall, this thesis enhances understanding of human-AI interaction and provides insights for developing AI systems across various applications.

==> fontsets/mitthesis-newtx-sans-text.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-newtx-sans-text.tex}[2023/10/03 v1.03 Load newtx sans-serif text and regular math fonts]

%% newtx package with sans-serif text (Helvetica-like text with Times-like math)
%
\ifpdftex
	\RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91,defaultsups]{newtx}% upint for upright integrals
	\AtEndPreamble{% added to accommodate v1.731 of newtx, 2023/11/03
	    \renewcommand{\familydefault}{\sfdefault}% use sans for main text
%	    \renewcommand{\rmdefault}{\sfdefault}% uses sans for \textrm{}, if that's desired.
	}
%   these two commands enable hyphenation of the typewriter font - https://tex.stackexchange.com/a/204421/119566
%    \input{t1ntxtt.fd}
%    \DeclareFontFamily{\encodingdefault}{\ttdefault}{\hyphenchar\font=`\-} % 
	\RequirePackage{bm}% bold math
\else
	\ClassWarning{mitnewthesis}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi

	

==> mydesign.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mydesign.tex}[2024/06/28 v1.04 Typographic design options for thesis]

%%%%%%%%%%  Color support  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Color package: xcolor. 
%% Change this if you prefer something else

\usepackage[dvipsnames,svgnames,x11names]{xcolor}

%% can add option [table] to xcolor to use color in tables (see xcolor documentation)


%%%%%%%%%%  Hyperlink and line number colors  %%%%%%%%%%%%%%

\AtBeginDocument{
    % Using color names from xcolor package
    \hypersetup{
    	linkcolor=Blue3,
    	citecolor=Blue3,
    	urlcolor=violet,
    	filecolor=red, 
    %	anchorcolor=yellow,%  not all pdf viewers recognize this field (although Firefox does): hyperref issues a warning
    %	colorscheme=phelype,% overrides link, cite, url, file colors with a preset scheme, through \DocumentMetadata
    	}
    %
    \ifmit@lineno
	    \renewcommand{\linenumberfont}{\sffamily\mdseries\tiny\color{violet}}% line numbers will be sans-serif, medium weight, tiny, and violet
	\fi
}

%%%%%%%%%  Caption support  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% see documentation for details of how to customize captions

\RequirePackage{caption}
\RequirePackage{subcaption}


%%%%%%%%%  Customize list environments  %%%%%%%%%%%%%%%%%%%%
% 
% see documentation for details of how to customize lists

%\RequirePackage{enumitem}


%%%%%%%%%  Customize titles and section headings  %%%%%%%%%%
% 
% see documentation for details of how to customize headings

\RequirePackage{titlesec}

% these titlesec commands just automate the bold math in some headings (rest follows default styles)
\titleformat{\section}{\mathversion{bold}\normalfont\Large\bfseries}{\thesection }{1em}{}
\titleformat{\subsection}{\mathversion{bold}\normalfont\large\bfseries}{\thesubsection}{1em}{}
\titleformat{\subsubsection}{\mathversion{bold}\normalfont\normalsize\bfseries}{\thesubsubsection}{1em}{}

% ==> NOT every font includes a bold math version, so you may need other math macros in the headings to get bold math <==


%%%%%%%%%  Change page margins  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% The default thesis margin is 1 inch all around. You may want different margins (e.g., to add a gutter for binding),
% in which case you can use the \newgeometry command from the geometry package.  Refer to the package documentation
% for details.
%
% mitthesis defaults: [top=1in,bottom=1in,left=1in,right=1in,marginparwidth=50pt,headsep=12pt,footskip=0.5in]
%
% The following tells the geometry package to use a two-sided layout with a 1 cm binding offset on the inside 
% 	and 1 inch margins all around, reducing textwidth slightly (by 0.7 cm). See geometry documentation, Section 8.2.
%
%\newgeometry{twoside, bindingoffset=1cm,margin=1in,marginparwidth=50pt,headsep=12pt,footskip=0.5in}

